Enhancing coastal water body segmentation with Landsat Irish Coastal Segmentation (LICS) dataset

Ireland's coastline, a critical and dynamic resource, is facing challenges such as erosion, sedimentation, and human activities. Monitoring these changes is a complex task we approach using a combination of satellite imagery and deep learning methods. However, limited research exists in this area, particularly for Ireland. This paper presents the Landsat Irish Coastal Segmentation (LICS) dataset, which aims to facilitate the development of deep learning methods for coastal water body segmentation while addressing modelling challenges specific to Irish meteorology and coastal types. The dataset is used to evaluate various automated approaches for segmentation, with U-NET achieving the highest accuracy of 95.0% among deep learning methods. Nevertheless, the Normalised Difference Water Index (NDWI) benchmark outperformed U-NET with an average accuracy of 97.2%. The study suggests that deep learning approaches can be further improved with more accurate training data and by considering alternative measurements of erosion. The LICS dataset and code are freely available to support reproducible research and further advancements in coastal monitoring efforts.

==> figures/all_mask_figures.tex <==

\begin{figure}[h]
\centering
\subfloat{
  \includegraphics[width=0.98\textwidth]{figures/205_23_masks.png}
  \label{fig:sub1}
} \vspace*{-1em}

\subfloat{
  \includegraphics[width=0.98\textwidth]{figures/205_24_masks.png}
  \label{fig:sub2}
} \vspace*{-1em}

%\subfloat{
  % \includegraphics[width=0.98\textwidth]{figures/206_22_masks.png}

%} \vspace*{-1em}

\subfloat{
   \includegraphics[width=0.98\textwidth]{figures/206_23_masks.png}

} \vspace*{-1em}

%\subfloat{
   %\includegraphics[width=0.98\textwidth]{figures/206_24_masks.png}

%} \vspace*{-1em}

\subfloat{
   \includegraphics[width=0.98\textwidth]{figures/207_22_masks.png}

} \vspace*{-1em}

%\subfloat{
   %\includegraphics[width=0.98\textwidth]{figures/207_23_masks.png}
%} \vspace*{-1em}

%\subfloat{
   %\includegraphics[width=0.98\textwidth]{figures/207_24_masks.png}

%} \vspace*{-1em}

%\subfloat{
  % \includegraphics[width=0.98\textwidth]{figures/208_22_masks.png}

%} \vspace*{-1em}

\subfloat{
   \includegraphics[width=0.98\textwidth]{figures/208_23_masks.png}

} \vspace*{-1em}

%\subfloat{
   %\includegraphics[width=0.98\textwidth]{figures/208_24_masks.png}
%} \vspace*{-1em}

\caption{Examples of predicted masks. Each row gives a random test image from a tile. The tile is given above the RGB visualisation in the first column. The second column gives the test mask for that image. The remaining 5 columns give the predicted mask for the 5 different approaches. The number next to the approach name gives the accuracy for that prediction when compared to the mask. The red line overlaying the predictions gives the edge of the coastline given in the mask. Examples for the remaining tiles can be found in the appendix.}

\label{fig:mask_examples}
\end{figure}

==> figures/metrics_altitude.tex <==
\begin{table}[ht]
\caption{Average accuracy by altitude category for the NDWI and UNET approaches. N gives the number of test images in each category. }
\label{tab:metrics_altitude}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Altitude} & \textbf{n} & \textbf{NDWI} & \textbf{UNET} \\ \hline
low               & 34         & 0.984         & 0.968         \\ \hline
medium            & 34         & 0.963         & 0.960         \\ \hline
high              & 32         & 0.969         & 0.968         \\ \hline
\end{tabular}
\end{table}

==> figures/metrics_clouds.tex <==
\begin{table}[ht]
\caption{Accuracy with clouds removed using Landsat CFMask algorithm. }
\label{tab:metrics_clouds}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Tile}  & \textbf{NDWI} & \textbf{UNET} \\ \hline
Original       & 0.972         & 0.966         \\ \hline
Clouds removed & 0.978         & 0.967         \\ \hline
\end{tabular}
\end{table}

==> figures/metrics_coastline.tex <==
\begin{table}[ht]
\caption{Evaluation metrics within 10 pixels of coastline. The average of the evaluation metrics over 100 test images is given.}
\centering
\label{tab:metrics_coastline}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    \\ \hline
NDWI            & \textbf{0.938}    & \textbf{0.983}     & 0.891           & \textbf{0.927} \\ \hline
XGBoost         & 0.845             & 0.875              & 0.816           & 0.825          \\ \hline
UNET            & 0.877             & 0.888              & 0.877           & 0.873          \\ \hline
ATTUNET         & 0.866             & 0.863              & \textbf{0.897}  & 0.872          \\ \hline
R2UNET          & 0.7               & 0.829              & 0.588           & 0.619          \\ \hline
\end{tabular}
\end{table}

==> figures/metrics_decade.tex <==
\begin{table}[ht]
\caption{Average accuracy by decade for the NDWI and UNET approaches. N gives the number of test images for each decade. }
\label{tab:metrics_decade}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Decade} & \textbf{N} & \textbf{NDWI} & \textbf{UNET} \\ \hline
1980            & 15         & 0.985         & 0.974         \\ \hline
1990            & 27         & 0.961         & 0.965         \\ \hline
2000            & 24         & 0.971         & 0.957         \\ \hline
2010            & 23         & 0.969         & 0.974         \\ \hline
2020            & 11         & 0.989         & 0.955         \\ \hline
\end{tabular}
\end{table}

==> figures/metrics_overall.tex <==
\begin{table}[ht]
\caption{Evaluation metrics for the segmentation approaches applied to the LICS test set. The average of the evaluation metrics over 100 test images is given. }
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1}      & \textbf{FOM}   \\ \hline
NDWI            & \textbf{0.972}    & \textbf{0.994}     & 0.946           & \textbf{0.967}        & \textbf{0.718} \\ \hline
XGBoost         & 0.927             & 0.945              & 0.88            & 0.897               & 0.483          \\ \hline
UNET            & 0.966             & 0.963              & 0.96            & 0.959                & 0.607          \\ \hline
ATTUNET         & 0.964             & 0.944              & \textbf{0.973}  & 0.956          & 0.591          \\ \hline
R2UNET          & 0.907             & 0.902              & 0.912           & 0.899                   & 0.34           \\ \hline
\end{tabular}

\label{tab:metrics_overall}
\end{table}



==> figures/metrics_tile.tex <==

\begin{table}[ht]
\caption{Average accuracy by tile for NDWI and U-NET. N gives the number of test images for each tile. }
\label{tab:metrics_tile}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Tile} & \textbf{N} & \textbf{NDWI} & \textbf{UNET} \\ \hline
(205,23)      & 11         & 0.990         & 0.954         \\ \hline
(205,24)      & 20         & 0.966         & 0.990         \\ \hline
(206,22)      & 9          & 0.982         & 0.981         \\ \hline
(206,23)      & 6          & 0.996         & 0.992         \\ \hline
(206,24)      & 10         & 0.976         & 0.943         \\ \hline
(207,22)      & 9          & 0.934         & 0.959         \\ \hline
(207,23)      & 10         & 0.991         & 0.968         \\ \hline
(207,24)      & 7          & 0.994         & 0.981         \\ \hline
(208,22)      & 6          & 0.959         & 0.972         \\ \hline
(208,23)      & 6          & 0.955         & 0.860         \\ \hline
(208,24)      & 6          & 0.943         & 0.983         \\ \hline
\end{tabular}

\end{table}

==> figures/tile_percentage.tex <==
\begin{table}[ht]
\caption{Percentage of test images that come from each tile in each decade.}
\label{tab:per_tiles}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Tile} & \textbf{1980} & \textbf{1990} & \textbf{2000} & \textbf{2010} & \textbf{2020} \\ \hline
(205,23)      & 7             & 15            & 8             & 13            & 9             \\ \hline
(205,24)      & 13            & 26            & 13            & 22            & 27            \\ \hline
(206,22)      & 7             & 7             & 4             & 17            & 9             \\ \hline
(206,23)      & 13            & 11            & 4             & 0             & 0             \\ \hline
(206,24)      & 7             & 7             & 13            & 17            & 0             \\ \hline
(207,22)      & 20            & 11            & 4             & 9             & 0             \\ \hline
(207,23)      & 13            & 11            & 8             & 9             & 9             \\ \hline
(207,24)      & 20            & 0             & 4             & 9             & 9             \\ \hline
(208,22)      & 0             & 0             & 25            & 0             & 0             \\ \hline
(208,23)      & 0             & 4             & 13            & 0             & 18            \\ \hline
(208,24)      & 0             & 7             & 4             & 4             & 18            \\ \hline
\end{tabular}
\end{table}
